LiST: Lite Prompted Self-training Makes Parameter-Efficient Few-shot Learners

We present a new method LiST is short for Lite Prompted Self-Training for parameter-efficient fine-tuning of large pre-trained language models (PLMs) for few-shot learning. LiST improves over recent methods that adopt prompt-based fine-tuning (FN) using two key techniques. The first is the use of self-training to leverage large amounts of unlabeled data for prompt-based FN in few-shot settings. We use self-training in conjunction with meta-learning for re-weighting noisy pseudo-prompt labels. Self-training is expensive as it requires updating all the model parameters repetitively. Therefore, we use a second technique for light-weight fine-tuning where we introduce a small number of task-specific parameters that are fine-tuned during self-training while keeping the PLM encoder frozen. Our experiments show that LiST can effectively leverage unlabeled data to improve the model performance for few-shot learning. Additionally, the fine-tuning is efficient as it only updates a small percentage of parameters and the overall model footprint is reduced since several tasks can share a common PLM encoder as backbone. A comprehensive study on six NLU tasks demonstrate LiST to improve by 35% over classic fine-tuning and 6% over prompt-based FN with 96% reduction in number of trainable parameters when fine-tuned with no more than 30 labeled examples from each task. With only 14M tunable parameters, LiST outperforms GPT-3 in-context learning by 33% on few-shot NLU tasks.

==> subfiles/back_up.tex <==

\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllll}
\toprule
\textbf{Examples} & \textbf{Models} & \multicolumn{1}{l}{\textbf{MNLI}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} & \multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}}  \\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 0$}
& BERT-base &  43.2/44.8 & 48.0 & 45.5/44.1
& 61.6 &  59.3 & 73.2 
\\

& BERT-large &45.0/46.0&50.5 & 38.1/49.5 &  61.2 & 63.6&68.0
\\

& RoBERTa-base  &48.3/49.4 & 53.4 & 40.5/51.6 & 77.8 &53.6 & 70.1\\

& RoBERTa-large  & 51.7/52.4 & 51.3 & 38.6/49.7 & 83.6 & 51.4 & 67.6

\\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 10$}
& BERT-base & 43.0 (2.1)/44.2 (2.1) &  52.5 (3.7) &59.6 (3.7)/26.0 (7.2)  & 70.9 (6.7) & 76.7 (10.5) &  63.7 (8.1) \\
& BERT-large & 44.5 (2.5)/45.7 (2.7) & 53.0 (1.8) & 54.0 (6.2)/32.8 (6.9) & 74.1 (7.9) & 77.6 (12.3) & 59.6 (5.3)\\
& RoBERTa-base  &  49.5 (2.9)/50.5 (3.1) & 56.4 (2.0) & 59.0 (4.1)/40.8 (9.4) & 85.7 (4.5) & 82.0 (6.7) & 67.8 (8.6)\\
& RoBERTa-large  & 54.8 (3.7)/55.6 (4.6) & 60.0 (4.4) & 58.7 (4.6)/41.2 (12.1)& 89.5 (1.7) & 84.5 (8.6) & 67.8 (6.9)\\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 20$}
& BERT-base  &  42.8 (2.1)/44.5 (2.8) &51.7 (3.3) & 62.3 (3.3)/30.3 (14.1) & 75.2 (6.6) & 84.2 (2.7) &  76.9 (5.3)

\\
& BERT-large&44.9 (2.6)/46.3 (3.2) & 51.6 (2.5) & 61.2 (3.8)/35.0 (10.7) & 77.9 (2.6) & 84.8 (2.5) & 75.3 (3.8) \\
& RoBERTa-base   & 51.9 (2.9)/52.8 (3.1) & 58.4 (4.0) & 66.1 (0.8)/43.4 (12.0)& 88.4 (0.8) & 88.1 (1.8) & 78.8 (4.3)\\
& RoBERTa-large & 60.3 (2.0)/61.6 (2.7) & 64.3 (2.4) & 67.8 (4.2)/43.9 (18.6) & 90.6 (1.8) &  88.3 (2.2) & 80.6 (7.5) \\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 30$}
& BERT-base &  44.7 (2.4)/45.7 (2.4) & 52.6 (4.0) & 62.6 (3.5)/39.7 (11.9)& 78.6 (3.8) & 85.1 (2.0) &  80.6 (2.7) \\

& BERT-large  & 47.6 (1.8)/48.7 (2.1) & 53.9 (3.5) & 60.4 (6.0)/44.6 (8.3) & 81.7 (3.8) & 86.2 (2.4) & 77.7 (2.2)\\

& RoBERTa-base  & 53.6 (2.4)/55.0 (3.0) & 61.0 (4.7) & 66.3 (2.9)/51.9 (5.5)& 89.1 (0.6) & 89.7 (2.1) & 81.6 (2.3)\\

& RoBERTa-large & 62.8 (2.6)/64.1 (3.3) & 66.1 (2.2) &  71.1 (1.5)/57.6 (9.2) & 91.5 (1.0)& 91.0 (0.5)&82.7 (3.8) \\

\midrule


\multirow{4}{*}{Full supervision}
& BERT-base  & 83.6 /84.1 & 64.6 & 91.1/88.0 & 91.1 &96.4 &  87.5

\\
& BERT-large & 86.0/85.7& 77.6 &91.6/88.7&93.2 &  97.2 &  88.2 

\\
& RoBERTa-base & 86.9/87.0 & 80.9 & 91.6/88.7& 93.7&97.0& 87.9 


\\
& RoBERTa-large & 89.3/88.8 & 88.4 & 92.1/89.4& 95.9& 97.1 & 89.3

 \\
 \midrule
 
\end{tabular}
}
\caption{Average accuracy and standard deviation for models on  MNLI, RTE, QQP, SST-2, Subj and MPQA for three training set sizes
$|\mathcal{T}|$. }
\label{fig:various_shot}
\end{table*}






\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllll}
\toprule
\textbf{Examples} & \textbf{Models} & \multicolumn{1}{l}{\textbf{MNLI}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} & \multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}}  \\
\midrule


\multirow{4}{*}{$|\mathcal{T}| = 10$}
& BERT-base & 32.1 (1.2)/32.4 (1.2) & 49.3 (2.6) & 60.3 (2.3)/23.6 (18.8) & 50.8 (3.4) & 69.4 (11.5) & 51.7 (2.2)
\\
& BERT-large & 35.7 (2.0)/35.5 (2.3) & 50.6 (6.1) & 62.3 (1.4)/25.1 (27.0) & 54.2 (6.5) &  68.5 (8.4) & 52.8 (4.3)
\\
& RoBERTa-base  & 35.2 (1.1)/35.3 (1.1) &50.6 (3.3) & 63.8 (0.9)/9.9 (9.6) & 49.9 (1.1)&74.4 (14.5)&51.4 (1.9)\\
& RoBERTa-large  & 34.9 (0.3)/35.2 (0.7)&50.3 (2.1)&61.1 (3.5)/17.7 (20.5)&51.8 (2.9)&71.2 (17.5)&52.4 (3.2)\\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 20$}
& BERT-base  & 33.1 (1.9)/33.4 (2.0) & 49.5 (5.4) &61.1 (5.9)/36.1 (15.1) & 57.6 (3.6) & 82.8 (3.1) &55.6 (6.2)


\\
& BERT-large& 35.7 (2.7)/36.0 (3.5)&50.6 (4.5)&62.6 (2.5)/30.6 (26.0) & 56.6 (4.5) & 81.5 (8.2) &55.6 (6.0)\\
& RoBERTa-base   &  36.1 (1.4)/36.5 (1.4) & 51.9 (4.5) & 61.0 (5.9)/21.6 (26.0) & 62.7 (8.4) & 86.0 (4.1) & 53.0 (5.3)\\
& RoBERTa-large &   35.8 (1.0)/36.8 (1.5) & 51.0 (4.8) & 61.3 (9.0)/30.2 (15.6) & 57.2 (7.7) & 84.8 (9.0) & 55.9 (4.1)
\\
\midrule

\multirow{4}{*}{$|\mathcal{T}| = 30$}
& BERT-base & 34.3 (2.0)/34.5 (1.9) & 51.6 (3.8) & 63.1 (3.6)/52.4 (4.3)&64.3 (12.0)&86.6 (5.1)&58.1 (6.1)\\
& BERT-large & 36.9 (3.2)/37.4 (3.6) & 52.1 (3.4) & 62.8 (1.8)/50.1 (14.9) & 59.4 (6.2) & 86.1 (4.9) & 57.4 (4.2)\\

& RoBERTa-base  & 38.2 (1.9)/38.6 (2.2) & 53.1 (2.4) & 62.5 (3.8)/42.9 (13.7) & 67.0 (10.3) & 87.5 (4.3) & 58.2 (7.2)\\

& RoBERTa-large & 38.0 (1.7)/39.0 (3.1) & 51.4 (3.7) &64.3 (8.1)/49.1 (8.1) & 65.0 (11.5) & 90.2 (2.2) &56.1 (5.3)\\

\midrule

\end{tabular}
}
\caption{Average accuracy and standard deviation for conventional FN models on  MNLI, RTE, QQP, SST-2, Subj and MPQA for three training set sizes
$|\mathcal{T}|$. }
\label{main_results}
\end{table*}


\begin{table}[hbt]

\centering
%\vspace{-0.1in}
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{l|lll}
\toprule
 \multirow{2}{*}{\textbf{Method}} &
\multicolumn{3}{c}{\textbf{Datasets}}\\
\cmidrule{2-4}
 & MNLI (m/mm) & RTE  & QQP \\
\midrule
\midrule
Few-shot Supervision & 62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} & 71.1 {\tiny(1.5)} / 57.6 {\tiny(9.2)} \\
PromptST  & 73.5 {\tiny(2.8)} / 75.0 {\tiny(3.7)} & 71.0 {\tiny(2.4)} & 75.2 {\tiny(0.9)} / 63.1 {\tiny(3.8)} \\
\midrule
PromptST w/o Adapter & 73.6 {\tiny(2.7)} / 74.8 {\tiny(2.7)} & 71.6 {\tiny(2.7)} & 74.6 {\tiny(1.5)} / 61.8 {\tiny(8.6)}\\
PromptST w/o FN stage\\
promptST w/o Warmup & 67.9 {\tiny(12.9)} / 69.0 {\tiny(13.1)} & 69.2 {\tiny(4.5)} & 72.4 {\tiny(5.8)} / 55.9 {\tiny(15.6)}
 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Pseudo-labeled Data Selection and Re-weighting Strategies}}\\
promptST w/o Re-weighting & 72.9 {\tiny(3.4)} / 74.2 {\tiny(4.5)} & 70.7 {\tiny(4.1)} & 74.5 {\tiny(1.2)} / 61.8 {\tiny(4.6)}
 \\
promptST w/ Hard Pseudo-Labels & 71.7 {\tiny(3.8)} / 73.0 {\tiny(5.4)}& 69.5 {\tiny (4.2)} \\
\bottomrule
\end{tabular}
}
\caption{Ablation analysis of our framework \sysname with 30 labeled examples  on MNLI, RTE and QQP.} 
\label{tab:ablation_model}
\end{table}



==> subfiles/exp_backup.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Experimental Setup}
\noindent\textbf{Dataset.} We perform large-scale experiments with six different natural language understanding tasks as summarized in Table~\ref{tab:datasets}. We use four tasks from GLUE~\citep{wang2019glue}, including MNLI~\citep{williams2018broad-mnli} for natural language inference, RTE~\citep{dagan2005pascal-rte1,bar2006second,giampiccolo2007third-rte3,bentivogli2009fifth-rte4} for textual entailment, QQP\footnote{\url{https://www.quora.com/q/quoradata/}} for semantic equivalence and SST-2~\citep{socher2013recursive-sst-2} for sentiment classification. The results are reported on their development set following~\citep{zhang2020revisiting}.  MPQA~\citep{wiebe2005annotating} and Subj~\citep{pang2004sentimental-subj} are used for polarity and subjectivity detection, where we follow~\citep{gao2021making} to keep $2,000$ examples for testing and use remaining examples for semi-supervised learning. 


For each dataset, we randomly sample $|\mathcal{K}| \in \{10, 20, 30\}$ manually labeled samples from the training data, and add the remaining to the unlabeled set while ignoring their labels -- following standard setups for semi-supervised learning. We repeatedly sample $K$ labeled instances five times, run each model with $5$ different seeds and report average performance with standard deviation across the runs. Furthermore, for every split and shot, we sample the labeled data such that $\mathcal{D}_{10}^{Train} \subset \mathcal{D}_{20}^{Train} \subset \mathcal{D}_{30}^{Train}$ to evaluate the impact of incremental sample injection. 

Following \textit{true few-shot learning} setting~\citep{perez2021true}, we do not use additional \textit{development set} beyond $|\mathcal{K}|$ labeled samples for hyper-parameter tuning or early stopping. The performance of each model is reported after fixed training epochs. \yq{The training epochs used in our experimental settings are presented in Appendix.}



\begin{table*}[t]
\begin{center}
\small
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{llcrccl}
\toprule
\textbf{Category} & \tf{Dataset} & \#Labels &  \tf{\#Full Train} & \tf{\#Test} & \tf{Type} & \tf{Labels} \\
\midrule
\multirow{3}{*}{\thead{sentence- \\pair  }} & MNLI & 3 &  392,702 & 9,815 & NLI & entailment, neutral, contradiction\\
& RTE & 2 &   2,490 & 277 & NLI &  entailment, not\_entailment \\
& QQP & 2 & 363,846 & 40,431 & paraphrase & equivalent, not\_equivalent  \\
\midrule
  \multirow{3}{*}{\thead{single-\\sentence }} & SST-2 & 2 &  6,920 & 872 & sentiment & positive, negative \\
 & Subj & 2 &  8,000 & 2,000 & subjectivity & subjective, objective \\
  & MPQA & 2 & 8,606 & 2,000 & opinion polarity & positive, negative \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Dataset summary and task descriptions. For each task, we sample $\mathcal{K} \in \{10, 20, 30\}$ labeled examples to form five different splits with different random seeds from the original training set, and add the remaining to the unlabeled set while ignoring their labels.}
\label{tab:datasets}
\end{table*}


\noindent\textbf{Baselines.} In addition to standard model tuning strategies, we also adopt several state-of-the-art semi-supervised methods as baselines including UST~\citep{mukherjee2020uncertainty}, MetaST~\citep{wang2021meta} and iPET~\citep{schick2021exploiting}. UST and MetaST are two self-training methods which are based on classic fine-tuning strategies. iPET is a semi-supervised method leveraging prompt fine-tuning strategy and ensemble approach to obtain state-of-the-art performance. We implement our framework in Pytorch and use Tesla V100 gpus for experiments. Hyper-parameter configurations  are presented in Appendix.


%In contrast to traditional semi-supervised setting, few-shot learning settings involve very few manually annotated training labels resulting in a noisy / weak model to start with. To handle this issue, we propose to introduce prompt fine-tuning into self-training to releash power of PLMs and overcome error propagation issue with a lightweight meta-learning adapter design, achieving data and parameter efficiency simultaneously. 





\subsection{Key Result}

%\noindent\textbf{Overall performance with few training labels.} 
Table~\ref{tab:main_results} shows the performance comparison among different models with $|\mathcal{K}| = 30$ labeled examples. Fully-supervised RoBERTa-large trained on thousands of labeled examples provides the ceiling performance for the few-shot setting. In Table~\ref{tab:main_results}, \sysname significantly outperforms other state-of-the-art baselines along with $96\%$ reduction in tunable parameters, achieving data and parameter efficiency simultaneously. More specifically, \sysname improves over Classic FN, Prompt FN and the best few-shot semi-supervised baseline iPET by $35.6\%$, $5.9\%$ and $9\%$ respectively in terms of average performance. This demonstrates the impact of self-training with unlabeled data and prompt-tuning. Additionally, iPET and \sysname both leverage prompt-tuning to significantly improve over UST and MetaST that use classic fine-tuning strategies, confirming the effectiveness of prompt-tuning in the low data regime.     

% \noindent\textbf{Performance with few training labels.}


\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllllll}
\toprule
\textbf{Labels} & \textbf{Models} & {\textbf{Avg}} & \textbf{\#Tunable} &\multicolumn{1}{l}{\textbf{MNLI (m/mm)}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} & \multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}} \\
&&&{\bf Params}&(acc) &(acc) &(acc/F1) & (acc)& (acc)&(acc)\\
\midrule

\multirow{2}{*}{\thead{$|\mathcal{K}| = 30$ }}

& Classic FN &59.7 &355M &38.0 {\tiny(1.7)} / 39.0 \tiny{(3.1)} & 51.4 {\tiny(3.7)} &64.3 {\tiny(8.1)}  & 65.0 {\tiny(11.5)} & 90.2 {\tiny(2.2)} &56.1 {\tiny(5.3)}\\
& Prompt FN & 76.5 &355M &62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} &  71.1 {\tiny(1.5)} & 91.5 {\tiny(1.0)} & 91.0 {\tiny(0.5)} &82.7 ({\tiny3.8)} \\

\midrule
\multirow{4}{*}{\thead{$|\mathcal{K}| = 30$ \\  +Unlabeled Data}}

&UST& \\
&MetaST& 61.0 & 355M &39.4 {\tiny(3.9)} / 40.5 {\tiny(4.4)} & 52.9 {\tiny(2.0)} & 65.7 {\tiny(6.2)} 
 & 65.3 {\tiny(15.2)}& 91.4 {\tiny(2.3)} & 60.5 {\tiny(3.6)}\\
&iPET & 74.3 & 355M&61.0 {\tiny(5.8)} / 61.8 {\tiny(4.7)} & 54.7 {\tiny(2.8)} & 67.3 {\tiny(4.1)}  & \textbf{93.8 {\tiny(0.6)}} & 92.6 {\tiny(1.5)}& 83.1 {\tiny(4.8)}\\
%& promptST-hard & 73.9 (3.6)/75.0 (3.5) &  & & 93.1 (0.8) & 92.0 (1.6) & \\
%&PromptST (Full) & 80.9  & 355M &\textbf{73.6 {\tiny(2.7)}} / 74.8 {\tiny(2.7)} & \textbf{71.6 {\tiny(2.7)}}  & 74.6 {\tiny(1.5)} / 61.8 {\tiny(8.6)}& 92.5 {\tiny(0.6)} & 92.4 {\tiny(0.5)}& \textbf{86.3 {\tiny(1.4)}}\\

% &&[$\uparrow$17.2\%/16.7\%] &  [$\uparrow$8.3\%] & [$\uparrow$4.9\%/7.3\%] & [$\uparrow$1.1\%] &[$\uparrow$1.5\%] & [$\uparrow$4.4\%]\\
% \midrule

 &PromptST& \textbf{81.0} &14M& 73.5 {\tiny(2.8)} / \textbf{75.0 {\tiny(3.7)}} &71.0 {\tiny(2.4)}&\textbf{75.2 {\tiny(0.9)} }& 92.8 {\tiny(0.9)} &\textbf{93.5 {\tiny(2.2)}} & 85.2 {\tiny(2.1)} \\
 \midrule
% \multirow{2}{*}{Supervision with  \# Full Train}
Supervision with & Classic FN & 90.7 & 355M & 89.6 / 89.5 &83.0& 91.8 &95.2&97.2&88.8 \\
\# Full Train & Prompt FN & 91.8 & 355M&89.3 / 88.8 & 88.4 & 92.1  & 95.9& 97.1 & 89.3

 \\
 \midrule
 
\end{tabular}
}
\caption{Performance comparison of different model tuning strategies on different tasks with RoBERTa-large as the encoder. UST, MetaST and iPET are semi-supervised methods using unlabeled data, whereas Classic and Prompt fine-tuning (FN) only use labeled data. The best performance is shown in \textbf{bold}.}
\label{tab:main_results}
\end{table*}

\begin{table*}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllllll}
\toprule
 \textbf{Models}  & \textbf{\#Params} &\textbf{Avg} &
\multicolumn{1}{l}{\textbf{MNLI (m/mm)}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} &
\multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}} \\
&&&(acc) &(acc) &(acc/F1) & (acc)& (acc)&(acc)\\
\midrule

BERT-base & 110M &65.5 &44.7 {\tiny(2.4)} / 45.7 {\tiny(2.4)} & 52.6 {\tiny(4.0)} & 62.6 {\tiny(3.5)} / 39.7 {\tiny(11.9)}& 78.6 {\tiny(3.8)} & 85.1 {\tiny(2.0)} &  80.6 {\tiny(2.7)} \\

BERT-large  &  336M  & 66.7&47.6 {\tiny(1.8)} / 48.7 {\tiny(2.1)} & 53.9 {\tiny(3.5)} & 60.4 {\tiny(6.0)} / 44.6 {\tiny(8.3)} & 81.7 {\tiny(3.8)} & 86.2 {\tiny(2.4)} & 77.7 {\tiny(2.2)}\\
\midrule
%\multirow{2}{*}{RoBERTa}
 RoBERTa-base  &125M & 72.5  &53.6 {\tiny(2.4)} / 55.0 {\tiny(3.0)} & 61.0 {\tiny(4.7)} & 66.3 {\tiny(2.9)} / 51.9 {\tiny(5.5)}& 89.1 {\tiny(0.6)} & 89.7 {\tiny(2.1)} & 81.6 {\tiny(2.3)}\\

 RoBERTa-large  & 355M & \textbf{76.5} &\textbf{62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)}} & \textbf{66.1 {\tiny(2.2)}} &  71.1 {\tiny(1.5)} / 57.6 {\tiny(9.2)} & 91.5 {\tiny(1.0)}& 91.0 {\tiny(0.5)}&82.7 {\tiny(3.8)}\\
	
	
\midrule
% \multirow{3}{*}{T5}

T5-small   & 60M & 63.9 &42.9 {\tiny(4.1)} / 44.0 {\tiny(5.0)} & 54.1 {\tiny(1.9)} & 56.7 {\tiny(4.2)} / 24.8 {\tiny(15.2)} &79.7 {\tiny(2.6)} & 85.0 {\tiny(1.8)} &  80.1 {\tiny(1.2)}\\



T5-base & 220M  & 69.5 &49.9 {\tiny(2.7)} / 51.4 {\tiny(3.5)} & 57.8 {\tiny(2.6)}  & 64.6 {\tiny(1.4)} / 35.8 {\tiny(11.4)}& 89.0 {\tiny(0.6)} &  88.9 {\tiny(2.1)} &  80.4 {\tiny(2.8)} 
\\

T5-large  &770M & 76.3 &57.3 {\tiny(5.9)} / 58.9 {\tiny(5.7)} & 61.6 {\tiny(3.0)} & \textbf{76.4 {\tiny(1.2)} / 64.8 {\tiny(5.5)}} &   \textbf{92.8 {\tiny(0.5)}} &  \textbf{91.0} {\tiny(1.6)} &  \textbf{83.6 {\tiny(1.4)}} \\


\midrule

 
\end{tabular}
}
\caption{Average performance and standard deviation of prompt-tuning with encoders of different sizes and families using only few-shot labeled data ($|\mathcal{K}|=30$).}
\label{tab:var_model}
\end{table*}




\begin{figure}[hbt!]
\vspace{-0.1in}
\subfloat[MNLI]{
\begin{minipage}{.34\linewidth}
\includegraphics[width=1.\linewidth]{./figures/mnli_trend}
\label{subfig:mnli}
\end{minipage}}
\subfloat[RTE]{
\begin{minipage}{.34\linewidth}
\includegraphics[width=1.\linewidth]{./figures/rte_trend}
\label{subfig:wnut17}
\end{minipage}}
\subfloat[Parameters]{
\begin{minipage}{.33\linewidth}
\includegraphics[width=1.\linewidth]{./figures/param_comparision}
\label{subfig:wnut17}
\end{minipage}}
 \caption{Performance changes of classic  tuning, prompt-tuning and PromptST    on   MNLI and RTE   tasks   for  a comparison.}\label{fig:threshold}
\end{figure}


% \begin{table*}
% \small
% \centering
% %\def\arraystretch{0.85}
% % \newcolumntype{Y}{>{\centering\arraybackslash}X}
% %\newcolumntype{a}{>{\columncolor{decentgrey}}c}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{clllllllll}
% \toprule
% \textbf{Examples} & \textbf{Models} & \multicolumn{1}{l}{\textbf{Average}}  &\multicolumn{1}{l}{\textbf{MNLI}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} & \multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}} \\
% \midrule

% {\thead{$|\mathcal{K}| = 30$ }}

% & Conventional FN &59.7  &38.0 (1.7)/39.0 (3.1) & 51.4 (3.7) &64.3 (8.1)/49.1 (8.1) & 65.0 (11.5) & 90.2 (2.2) &56.1 (5.3)\\
% & Prompt FN & 76.5 &62.8 (2.6)/64.1 (3.3) & 66.1 (2.2) &  71.1 (1.5)/57.6 (9.2) & 91.5 (1.0)& 91.0 (0.5)&82.7 (3.8) \\

% \midrule
% \multirow{6}{*}{\thead{$|\mathcal{K}| = 30$ \\  +Unlabeled Data}}

% &UST& \\
% &MetaST& &36.6 (2.8)/37.6 (4.3) & 52.9 (2.0) & 63.2 (0.1)/6.9 (15.4) & 65.3 (15.2)& 91.4 (2.3) & 60.5 (3.6)\\
% &iPET & 74.3 & 61.0 (5.8)/61.8 (4.7) & 54.7 (2.8) & 67.3 (4.1)/52.9 (6.5) & \textbf{93.8 (0.6)} & 92.6 (1.5)& 83.1 (4.8)\\
% %& promptST-hard & 73.9 (3.6)/75.0 (3.5) &  & & 93.1 (0.8) & 92.0 (1.6) & \\

% &PromptST & 80.9   &\textbf{73.6 (2.7)}/74.8 (2.7) & \textbf{71.6 (2.7)}  & 74.6 (1.5)/61.8 (8.6)& 92.5 (0.6) & 92.4 (0.5)& \textbf{86.3 (1.4)}\\
% % &&[$\uparrow$17.2\%/16.7\%] &  [$\uparrow$8.3\%] & [$\uparrow$4.9\%/7.3\%] & [$\uparrow$1.1\%] &[$\uparrow$1.5\%] & [$\uparrow$4.4\%]\\
% % \midrule

%  &PromptST-Adapter(4\%)& \textbf{81.0} & 73.5 (2.8)/\textbf{75.0 (3.7)} &71.0 (2.4)&\textbf{75.2 (0.9)/63.1} (3.8)& 92.8 (0.9) &\textbf{93.5 (2.2)} & 85.2 (2.1) \\

%  &PromptSTA(4\%)& \textbf{81.0} & 73.5 (2.8)/\textbf{75.0 (3.7)} &71.0 (2.4)&\textbf{75.2 (0.9)/63.1} (3.8)& 92.8 (0.9) &\textbf{93.5 (2.2)} & 85.2 (2.1) \\
%  \midrule
% \multirow{1}{*}{Full supervision}

% & Prompt FN & 91.8 & 89.3/88.8 & 88.4 & 92.1/89.4 & 95.9& 97.1 & 89.3

%  \\
%  \midrule
 
% \end{tabular}
% }
% \caption{Average accuracy and standard deviation for models on SST-2, Subj, MPQA, MNLI, RTE and QQP.  The improvement is over  RoBERTa-large with labeled data
% $|\mathcal{K}|$.}
% \label{tab:main_results}
% \end{table*}



\subsection{Few-shot Supervision}

To better understand the role of different model families in few-shot learning, we evaluate the performance of representative state-of-the-art PLMs like BERT~\citep{BERT}, RoBERTa~\citep{RoBERTa} and T5~\citep{T5} of different sizes (parameters) with varying amounts of labeled data. %First, we compare the performance of PLMs  model with different checkpoint sizes. Then, we evaluate the performance of one PLM with different size of labeled data from 10 to 30 to study effect of labeled samples. 
We report macro-averaged results for each model trained on five different splits and macro-averaged results over six tasks for easy comparison.



\noindent\textbf{Effect of model choices.}  Table~\ref{tab:var_model} shows the performance comparison of three representative PLMs with different parameters with $30$ labeled samples. We observe that average performance increases with increase in model sizes within each model family. %The performance comparison of different model families shows that model family is a very important factor. 
%As shown in Table~\ref{tab:var_model}, RoBERTa-base brings 8.7\% average performance improvement over BERT-large using only 37\% parameters, confirming the importance of 
%pre-training stage for few-shot scenario. Moreover, RoBERTa-large outperforms all the other PLMs including T5-large with more parameters. 
Overall, we observe RoBERTa models to perform much better than BERT, and marginally outperform T5 models of much bigger size. Accordingly, we use RoBERTa-large as the base encoder for both \sysname and other baseline methods. 








\noindent\textbf{Effect of varying the number of labels $|\mathcal{K}|$.} %Since RoBERTa-large outperforms other PLMs, we adopt RoBERTa-large as backbone to study effects of varying number of labels.  
Table~\ref{tab:var_shot} shows the performance comparison of RoBERTa-large with classic and prompt-tuning strategies and varying the number of labeled samples (shots) including zero-shot supervision, few-shot and full supervision. Prompt-tuning works well even in the zero-shot setting and outperforms classic tuning across all settings. With increase in the amount of labeled examples, prompt-tuning significantly improves in performance outperforming classic tuning. With full supervision, however, both the strategies obtain a similar performance. This demonstrates prompt-tuning to be the most impactful for low-resource settings with few training labels for a given task.






\subsection{Adapter}
\label{subsec:adapter}

In this section, we explore several choices of adapter design for prompt-tuning for few-shot learning with RoBERTa-large as encoder. %First, we conduct pilot studies to identify  important modules in few-shot supervision for adapter placement. Then we evaluate the performance of the proposed Prompt Adapter in few-shot supervision with a comparison to other state-of-the-art lightweight fine-tuning baselines. 


\noindent\textbf{Where to insert an adapter in Transformers?} In order to answer this question, we conduct an experiment to study the role of various Transformer modules in few-shot prompt-tuning. To this end, we tune a given module along with the language model head while keeping all other parameters frozen. % following recent lightweight studies~\citep{pfeiffer2020AdapterHub}. 
Table~\ref{tab:adapter_pilot} shows the performance comparison of tuning specific modules on six tasks with varying number of labeled examples. The main modules of RoBERTa include \textit{Embedding}, \textit{Attention}, \textit{Feedforward Output} and \textit{Feedforward Intermediate} layers. We observe that tuning only the \textit{Feedforward Output} or the \textit{Attention} module delivers the best performance across most tasks with few-shot labels. Correspondingly, this motivated us to insert our adapter parameters into these two modules.  %For some tasks, Attention modules achieve best performance. Such observations motivate us to insert Adapter into \textit{Feedforward Output} and \textit{Attention} modules to handle diverse tasks. 


\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllllll}
\toprule
\textbf{Labels} &  \textbf{Tuning} & \textbf{\#Params} &  \textbf{Avg} & {\textbf{MNLI (m/mm)}}  & {\textbf{RTE}}   & {\textbf{QQP}} & {\textbf{SST-2}} & {\textbf{Subj}} & {\textbf{MPQA}} \\
&&&&(acc) &(acc) &(acc/F1) & (acc)& (acc)&(acc)\\
\midrule


\multirow{4}{*}{$|\mathcal{K}| = 10$}
& Full  & 355M&67.8&54.8 {\tiny(3.7)} / 55.6 {\tiny(4.6)} & 60.0 {\tiny(4.4)} & 58.7 {\tiny(4.6)} / 41.2 {\tiny(12.1)}& 89.5 {\tiny(1.7)} & 84.5 {\tiny(8.6)} & 67.8 {\tiny(6.9)}\\

& Embedding & 53M&60.4&53.3 {\tiny(1.1)} / 53.7 {\tiny(1.2)}& 56.1 {\tiny(3.5)} & 50.9 {\tiny(6.4)} / 28.2 {\tiny(9.9)}&84.4 {\tiny(3.6)}&70.3 {\tiny(6.0)}&58.8 {\tiny(7.0)} \\
& Attention & 101M&66.6 &55.1 {\tiny(3.0)} / 55.8 {\tiny(4.0)} & 57.9 {\tiny(3.9)}& 57.8 {\tiny(7.0)} / 41.8 {\tiny(9.2)} & 90.3 {\tiny(1.5)} &82.0 {\tiny(6.6)} &64.3 {\tiny(6.6)}
\\
& FF-output & 102M& 67.7&55.7 {\tiny(3.3)} / 56.4 {\tiny(4.0)} &60.4 {\tiny(4.3)} & 59.1 {\tiny(5.7)} / 43.0 {\tiny(4.2)} & 90.2 {\tiny(1.5)} & 82.2 {\tiny(7.1)} & 66.2 {\tiny(8.1)} \\
& FF-intermediate &102M &65.8&55.0 {\tiny(2.8)} / 55.7 {\tiny(3.7)} & 57.7 {\tiny(3.5)} & 57.0 {\tiny(7.2)} / 41.5 {\tiny(5.5)}
& 89.3 {\tiny(2.1)} & 80.7 {\tiny(6.1)} & 62.7 {\tiny(6.9)} \\

\midrule

\multirow{4}{*}{$|\mathcal{K}| = 20$}

& Full &355M &73.4&60.3 {\tiny(2.0)} / 61.6 {\tiny(2.7)} & 64.3 {\tiny(2.4)} & 67.8 {\tiny(4.2)} / 43.9 {\tiny(18.6)} & 90.6 {\tiny(1.8)} &  88.3 {\tiny(2.2)} & 80.6 {\tiny(7.5)} \\
& Embedding & 53M&63.1&53.2 {\tiny(1.3)} / 53.1 {\tiny(1.5)} & 58.1 {\tiny(0.9)} & 55.7 {\tiny(5.2)} / 25.0 {\tiny(13.4)} & 86.0 {\tiny(1.7)} & 78.0 {\tiny(2.0)} & 62.7 {\tiny(3.2)} \\
& Attention &101M &72.6&59.2 {\tiny(1.7)} / 60.2 {\tiny(2.4)} &  61.4 {\tiny(2.2)} & 66.8 {\tiny(2.6)} / 43.0 {\tiny(16.8)} & 91.7 {\tiny(1.1)} &  88.6 {\tiny(1.5)} & 79.3 {\tiny(5.5)}
\\

& FF-output& 102M&73.9&60.2 {\tiny(1.8)} / 61.4 {\tiny(2.6)} & 65.2 {\tiny(2.5)} & 67.7 {\tiny(3.4)} / 46.8 {\tiny(13.4)} & 91.4 {\tiny(1.4)} &  88.5 {\tiny(1.3)} & 80.3 {\tiny(5.2)}

 \\
& FF-intermediate &102M &71.7&58.3 {\tiny(1.6)} / 59.3 {\tiny(2.0)} & 60.8 {\tiny(2.3)} & 66.2 {\tiny(3.2)} / 44.6 {\tiny(13.3)} & 90.5 {\tiny(1.3)} & 87.4 {\tiny(2.3)} & 77.4 {\tiny(5.8)} \\

\midrule

\multirow{4}{*}{$|\mathcal{K}| = 30$}

& Full & 355M &76.5&62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} &  71.1 {\tiny(1.5)} / 57.6 {\tiny(9.2)} & 91.5 {\tiny(1.0)}& 91.0 {\tiny(0.5)} &82.7 {\tiny(3.8)}\\
& Embedding &53M &64.9&54.1 {\tiny(1.1)} / 54.0 {\tiny(1.2)} & 59.0 {\tiny(2.7)}  & 56.7 {\tiny(4.5)} / 31.7 {\tiny(6.6)} &  85.8 {\tiny(0.9)} & 82.2 {\tiny(2.6)} & 64.2 {\tiny(2.1)} \\
& Attention &101M & 76.0&61.6 {\tiny(2.2)} / 62.7 {\tiny(2.9)} & 65.8 {\tiny(3.2)} & 70.1 {\tiny(2.2)} / 57.0 {\tiny(6.0)} & 91.7 {\tiny(0.9)} & 90.4 {\tiny(0.7)} & 82.1 {\tiny(2.5)}\\
& FF-output & 102M&76.5&62.3 {\tiny(2.1)} / 63.5 {\tiny(3.0)} & 67.3 {\tiny(2.6)} &  70.8 {\tiny(1.7)} / 58.3 {\tiny(4.0)} & 91.8 {\tiny(0.8)} & 90.2 {\tiny(1.3)} & 82.5 {\tiny(3.4)}

\\
& FF-intermediate  &102M & 74.9& 60.4 {\tiny(1.9)} / 61.4 {\tiny(2.5)} & 64.0 {\tiny(3.9)} &  69.0 {\tiny(2.7)} / 56.1 {\tiny(5.1)} & 91.0 {\tiny(1.2)} & 90.0 {\tiny(1.3)} &80.7 {\tiny(2.7)}

\\


\midrule

 
\end{tabular}
}
\caption{Average performance and standard deviation on tuning different modules of RoBERTa-large with varying amount of training labels $|\mathcal{K}|$.}
\label{tab:adapter_pilot}
\end{table*}



\noindent\textbf{Comparison with other lightweight parameter-efficient model tuning strategies.} To validate the effectiveness of the \sysname adapters, we compare it to several state-of-the-art baselines including Bias-only~\citep{cai2020tinytl},  Head-only, and Houlsby Adapter~\citep{houlsby2019parameter}. \yq{(1) Bias-only is a simple but effective lightweight method, which tunes bias terms of PLMs while keeping other parameters frozen. (2) Tuning head layers is widely used as a strong baseline for lightweight studies. In this work, we tune last two layers of language model head while freezing other parameters.  (3) Houlsby Adapter is to tune inserted adapter only with other parameters frozen. Such a method is a state-of-the-art lightweight tuning method based on classic tuning.}
Besides these lightweight methods, we also present a performance comparison with full model tuning as a strong baseline.  








\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{clll}
\toprule
\textbf{Bottleneck Dim}  & \textbf{\#Params} &  \multicolumn{1}{l}{\textbf{MNLI (m/mm)}}  & \multicolumn{1}{l}{\textbf{RTE}}    \\
& &(acc) &(acc) \\
\midrule

2& 1M  &56.6 {\tiny(3.5)} / 57.4 {\tiny(4.1)} & 64.0 {\tiny(4.2)}\\
8 & 2M &57.8 {\tiny(3.7)} / 58.9 {\tiny(4.4)} & 65.4 {\tiny(3.4)}\\
32 & 4M &60.5 {\tiny(3.7)} / 61.9 {\tiny(4.6)} & 65.9 {\tiny(3.4)}\\
128 & 14M  &62.4 {\tiny(1.7)} / 63.7 {\tiny(2.5)} & 66.6 {\tiny(3.9)} \\
512 & 51M &63.4 {\tiny(3.8)} / 64.6 {\tiny(4.7)} & 67.5 {\tiny(3.9)}\\


\midrule

\end{tabular}
}
\caption{Performance comparison of \sysname adapter with various bottleneck dimensions. }
\label{tab:var_bottleneck}
\end{table*}


\begin{table*}
\small
\centering
%\def\arraystretch{0.85}
% \newcolumntype{Y}{>{\centering\arraybackslash}X}
%\newcolumntype{a}{>{\columncolor{decentgrey}}c}
\resizebox{\textwidth}{!}{
\begin{tabular}{llclllllll}
\toprule
 \textbf{Tuning} & \textbf{\#/\%  Params}& \textbf{Avg} & \multicolumn{1}{c}{\textbf{MNLI (m/mm)}}  & \multicolumn{1}{c}{\textbf{RTE}}   & \multicolumn{1}{c}{\textbf{QQP}} & \multicolumn{1}{c}{\textbf{SST-2}} & \multicolumn{1}{c}{\textbf{Subj}} & \multicolumn{1}{c}{\textbf{MPQA}} \\
\midrule


 Head-only &1M& 64.8&54.1 {\tiny(1.1)} / 54.1 {\tiny(1.3)} & 58.8 {\tiny(2.6)} & 56.7 {\tiny(4.5)} / 31.6 {\tiny(6.6)} & 85.6 {\tiny(1.0)}& 82.1 {\tiny(2.5)} & 64.1 {\tiny(2.1)} \\
 Bias-only& 1M & 66.3& 54.4 {\tiny(1.3)} / 54.4 {\tiny(1.5)}& 59.8 \tiny{(3.5)} & 58.6 {\tiny(4.4)} / 34.5 {\tiny(6.5)} & 87.3 {\tiny(1.1)} & 83.9 {\tiny(2.3)}& 65.8 {\tiny(1.8)}  \\
 
 Prompt-only &1M/0.3\%& 56.7 & 47.3 {\tiny(0.2)} / 47.7 {\tiny(0.1)} & 53.0 {\tiny(0.6)} &39.9 {\tiny(0.7)} / 43.5 {\tiny(1.5)} & 75.7 {\tiny(1.7)} & 51.5 {\tiny(1.4)} & 70.9 {\tiny(2.4)}
 
  \\
 
  Houlsby Adapter &14M/3.9\%& 55.7& 35.7 {\tiny(1.1)} / 36.2 {\tiny(2.0)} & 51.0 {\tiny(3.0)} & 62.8 {\tiny(3.0)} / 37.1 {\tiny(11.9)} & 57.0 {\tiny(6.2)} & 83.2 {\tiny(5.4)} & 57.2 {\tiny(3.5)}

\\
 \sysname Adapter  & 14M/3.9\% & \textbf{76.7}& \textbf{62.4 {\tiny(1.7)} / 63.7 {\tiny(2.5)}} &\textbf{66.6 {\tiny(3.9)}}&\textbf{71.2 {\tiny(2.6)} / 59.0 {\tiny(4.0)}}&\textbf{91.7 {\tiny(1.0)}} & \textbf{90.9 {\tiny(1.3)}} & \textbf{82.6 {\tiny(2.0)}}
 \\ 
 \midrule
  Full tuning & 355M/100\% &76.5&62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} &  71.1 {\tiny(1.5)} / 57.6 {\tiny(9.2)} & 91.5 {\tiny(1.0)}& 91.0 {\tiny(0.5)} &82.7 {\tiny(3.8)}\\

\midrule
 
\end{tabular}
}
\caption{Average performance and standard deviation of several lightweight parameter-efficient prompt-tuning strategies with $|\mathcal{K}| = 30$ training labels. The best performance is shown in \textbf{bold} along with the number ($\#$) of adapter parameters and the percentage ($\%$) of total encoder parameters. }

\label{tab:adapter}
\end{table*}


\subsection{Ablation Analysis}
Table~\ref{tab:ablation_model} demonstrates the impact of different components and design choices of \sysname with ablation analysis. 

\noindent$\bullet$ \textbf{Adapter training stability.} Training with very few training labels without any additional development set results in instability for few-shot adapter training. To demonstrate training stability, we include the average accuracy and standard deviation across several runs and splits as metrics. We observe that hard pseudo-labels hurt the model performance compared to soft pseudo-labels and exacerbate the instability issue. This is in contrast to observations from classic fine-tuning~\citep{}. A potential reason could be the use of a well pre-trained language model head for prompt-tuning that is able to indicate meaningful relationships among different prompt labels. 



\noindent$\bullet$ \textbf{PromptST versus PromptST w/o Adapter.} In {\tt PromptST}, we only fine-tune the adapter and language model head while keeping other encoder parameters frozen to achieve parameter efficiency. %Even though Prompt Adapter design shows similar performance with that of full model with few-shot supervision, we conduct ablation study to compare adapter and full model choices in few-shot semi-supervised learning setting.
Table~\ref{tab:ablation_model} shows that \sysname using only $4\%$ tunable parameters is able to match the performance of fully tunable \sysname (that is without using any adapters) on MNLI and RTE -- demonstrating the effectiveness of our lightweight design.  

\noindent$\bullet$ \textbf{Knowledge Distillation Warmup.} In this ablation study, we remove the warmup phase with knowledge distillation from {\tt PromptST} (denoted as ``PromptST w/o KD Warmup''). Removing this component leads to around $4\%$ performance drop in terms of average accuracy and $300\%$ larger standard deviation -- demonstrating the importance of KD Warmup in stabilizing {\tt PromptST} training.





% \begin{table}[hbt]

% \centering
% %\vspace{-0.1in}
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{l|lll}
% \toprule
%  \multirow{2}{*}{\textbf{Method}} &
% \multicolumn{3}{c}{\textbf{Datasets}}\\
% \cmidrule{2-4}
%  & MNLI (m/mm) & RTE  & QQP \\
% \midrule
% \midrule
% Few-shot Supervision & 62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} & 71.1 {\tiny(1.5)} / 57.6 {\tiny(9.2)} \\
% PromptST  & 73.5 {\tiny(2.8)} / 75.0 {\tiny(3.7)} & 71.0 {\tiny(2.4)} & 75.2 {\tiny(0.9)} / 63.1 {\tiny(3.8)} \\
% \midrule
% PromptST w/o Adapter & 73.6 {\tiny(2.7)} / 74.8 {\tiny(2.7)} & 71.6 {\tiny(2.7)} & 74.6 {\tiny(1.5)} / 61.8 {\tiny(8.6)}\\
% PromptST w/o FN stage\\
% promptST w/o Warmup & 67.9 {\tiny(12.9)} / 69.0 {\tiny(13.1)} & 69.2 {\tiny(4.5)} & 72.4 {\tiny(5.8)} / 55.9 {\tiny(15.6)}
%  \\
% % \midrule
% % \multicolumn{3}{l}{\textbf{Pseudo-labeled Data Selection and Re-weighting Strategies}}\\
% promptST w/o Re-weighting & 72.9 {\tiny(3.4)} / 74.2 {\tiny(4.5)} & 70.7 {\tiny(4.1)} & 74.5 {\tiny(1.2)} / 61.8 {\tiny(4.6)}
%  \\
% promptST w/ Hard Pseudo-Labels & 71.7 {\tiny(3.8)} / 73.0 {\tiny(5.4)}& 69.5 {\tiny (4.2)} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation analysis of our framework \sysname with 30 labeled examples  on MNLI, RTE and QQP.} 
% \label{tab:ablation_model}
% \end{table}



\begin{table}[hbt]

\centering
%\vspace{-0.1in}
\resizebox{0.7\columnwidth}{!}{
\begin{tabular}{lcclll}
\toprule
 \multirow{2}{*}{\textbf{Method}} &  \multirow{2}{*}{\textbf{Avg Acc}} & \multirow{2}{*}{\textbf{Avg Std}} & 
\multicolumn{3}{c}{\textbf{Datasets}}\\
\cmidrule{4-6}
 & && MNLI (m/mm) & RTE   \\
\midrule
\midrule
Prompt-tuning &64.8 & 2.6 & 62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)} & 66.1 {\tiny(2.2)} \\
PromptST  & 72.6 &2.8 & 73.5 {\tiny(2.8)} / 75.0 {\tiny(3.7)} & 71.0 {\tiny(2.4)} \\
\midrule
Vanilla Prompt Self-training & 55.6&1.6& 53.9 {\tiny(0.6)} / 54.3 {\tiny(0.7)} & 57.0 {\tiny(2.6)}\\
PromptST w/o Adapter & 72.6 & 2.5 & 73.6 {\tiny(2.7)} / 74.8 {\tiny(2.7)} & 71.2 {\tiny(2.3)}\\
PromptST w/o FN stage & \\
promptST w/o KD Warmup & 68.8 & 8.8 &67.9 {\tiny(12.9)} / 69.0 {\tiny(13.1)} & 69.2 {\tiny(4.5)} 
 \\
% \midrule
% \multicolumn{3}{l}{\textbf{Pseudo-labeled Data Selection and Re-weighting Strategies}}\\
promptST w/o Re-weighting &  71.6 & 4.0&72.9 {\tiny(3.4)} / 74.2 {\tiny(4.5)} & 69.7 {\tiny(4.1)} 
 \\
promptST w/ Hard Pseudo-Labels & 70.9 & 4.4 &71.7 {\tiny(3.8)} / 73.0 {\tiny(5.4)}& 69.5 {\tiny (4.2)} \\
\bottomrule
\end{tabular}
}
\caption{Ablation analysis of \sysname with 30 labeled examples on MNLI and RTE.} 
\label{tab:ablation_model}
\end{table}




\begin{table*}
\small
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{clllllllll}
\toprule
 \textbf{Models}  & \textbf{\#Params} &\textbf{Avg} &
\multicolumn{1}{l}{\textbf{MNLI (m/mm)}}  & \multicolumn{1}{l}{\textbf{RTE}}   & \multicolumn{1}{l}{\textbf{QQP}} &
\multicolumn{1}{l}{\textbf{SST-2}} & \multicolumn{1}{l}{\textbf{Subj}} & \multicolumn{1}{l}{\textbf{MPQA}} \\
&&&(acc) &(acc) &(acc) & (acc)& (acc)&(acc)\\
\midrule

BERT-base & 110M & 67.4 &44.7 {\tiny(2.4)} / 45.7 {\tiny(2.4)} & 52.6 {\tiny(4.0)} & 62.6 {\tiny(3.5)} & 78.6 {\tiny(3.8)} & 85.1 {\tiny(2.0)} &  80.6 {\tiny(2.7)} \\

BERT-large  &  336M  & 68.0&47.6 {\tiny(1.8)} / 48.7 {\tiny(2.1)} & 53.9 {\tiny(3.5)} & 60.4 {\tiny(6.0)} & 81.7 {\tiny(3.8)} & 86.2 {\tiny(2.4)} & 77.7 {\tiny(2.2)}\\
\midrule
%\multirow{2}{*}{RoBERTa}
 RoBERTa-base  &125M & 73.7  &53.6 {\tiny(2.4)} / 55.0 {\tiny(3.0)} & 61.0 {\tiny(4.7)} & 66.3 {\tiny(2.9)} & 89.1 {\tiny(0.6)} & 89.7 {\tiny(2.1)} & 81.6 {\tiny(2.3)}\\

 RoBERTa-large  & 355M & \textbf{77.6} &\textbf{62.8 {\tiny(2.6)} / 64.1 {\tiny(3.3)}} & \textbf{66.1 {\tiny(2.2)}} &  71.1 {\tiny(1.5)}  & 91.5 {\tiny(1.0)}& 91.0 {\tiny(0.5)}&82.7 {\tiny(3.8)}\\
	
	
\midrule
% \multirow{3}{*}{T5}

T5-small   & 60M & 66.5 &42.9 {\tiny(4.1)} / 44.0 {\tiny(5.0)} & 54.1 {\tiny(1.9)} & 56.7 {\tiny(4.2)}  &79.7 {\tiny(2.6)} & 85.0 {\tiny(1.8)} &  80.1 {\tiny(1.2)}\\



T5-base & 220M  & 71.9 &49.9 {\tiny(2.7)} / 51.4 {\tiny(3.5)} & 57.8 {\tiny(2.6)}  & 64.6 {\tiny(1.4)} & 89.0 {\tiny(0.6)} &  88.9 {\tiny(2.1)} &  80.4 {\tiny(2.8)} 
\\

T5-large  &770M & 77.3 &57.3 {\tiny(5.9)} / 58.9 {\tiny(5.7)} & 61.6 {\tiny(3.0)} & \textbf{76.4 {\tiny(1.2)} } &   \textbf{92.8 {\tiny(0.5)}} &  \textbf{91.0} {\tiny(1.6)} &  \textbf{83.6 {\tiny(1.4)}} \\


\midrule

 
\end{tabular}
}
\caption{Average performance and standard deviation of prompt-tuning with encoders of different sizes and families using only few-shot labeled data ($|\mathcal{K}|=30$).}
\label{tab:var_model}
\end{table*}


==> subfiles/introduction.tex <==
          \section{Introduction}

Large pre-trained language models (PLMs) have obtained state-of-the-art performance in several natural language understanding tasks~\citep{DBLP:conf/naacl/DevlinCLT19,DBLP:conf/iclr/ClarkLLM20,DBLP:journals/corr/abs-1907-11692}. Despite their remarkable success, these large language models suffer from two significant challenges. 

\noindent {\em (C1) Labeled training data.} PLMs traditionally rely on thousands of labeled training data for adapting to downstream tasks to obtain state-of-the-art performance. While models like GPT-3~\citep{brown2020language} have obtained impressive few-shot performance with in-context task adaptation, they have a significant performance gap relative to fully supervised SOTA models. For instance, the few-shot GPT-3 performance is $20$ points worse than the fully-tuned DeBERTa~\citep{DBLP:conf/iclr/HeLGC21} on SuperGLUE. This poses significant challenges for many real-world tasks where large labeled data is difficult to obtain. 

\noindent {\em (C2) Large number of tunable parameters.} PLMs have been steadily increasing in size in terms of trainable parameters ranging from millions to billions of parameters. %{ With increasing number of parameters, few-shot leanring performance of large models have been improving, achieving better
%performance with fewer optimization steps and data points~\citep{kaplan2020scaling}. 
%However, to reach state-of-the-art performance, they still require adaption, for instance, by fine-tuning all the parameters on task-specific labeled data. 
This significantly increases both the computational cost to fine-tune all parameters of the very large PLM and the serving cost in terms of the storage and overall model footprint, where every task requires its customized copy of the large model parameters. 
%
%\xiaodl{Can we find some references for both C1/C2?}
%
In order to address the above challenges, we consider real-world settings where fine-tuning PLMs needs to meet the following two criteria.

\begin{itemize}
    \item Few-shot: We assume very limited amount of task labels in each task domain.
    \item Light-weight: The fine-tuning should have a small number of tunable parameters, for each new task, to reduce the overall storage cost and model footprint.
\end{itemize}

Note that the computational cost of inference is out of the scope of this paper and previous work has studied several ways to address it including model distillation~\citep{hinton2015distilling}, pruning~\citep{lecun1990optimal}, etc. 

In this work, we present a new fine-tuning method \sysname that aims to improve  few-shot learning ability and parameter-efficiency over existing fine-tuning strategies using two key techniques:


\begin{figure}[hbt!]
\vspace{-0.3in}
\subfloat[Performance Comparison]{
\begin{minipage}{.49\linewidth}
\includegraphics[width=1.0\linewidth]{figures/open_fig1}\vspace{-0.15in}
\label{subfig:mnli}
\end{minipage}}
\subfloat[Tunable Parameters]{
\begin{minipage}{.49\linewidth}
\includegraphics[width=1.0\linewidth]{./figures/open_fig2}\vspace{-0.15in}
\label{subfig:rte}
\end{minipage}}

 \caption{\sysname leverages prompt-based fine-tuning (FN) with unlabeled data for label-efficiency and adapters for reducing tunable parameters . (a) shows classic tuning, prompt-based FN and \sysname using RoBERTa-large as backbone on MNLI task for a comparison. The red dash line depicts the ceiling performance with full supervision  with RoBERTa-large.  (b) shows the number of tunable parameters for each method. Table~\ref{tab_app:gpt-3} shows a comparison with GPT-3 in-context learning. }\label{fig:key-result}\vspace{-0.1in}
\end{figure}


\noindent {\em (a) Self-training with prompts and unlabeled data.} The first one is to leverage self-training with large amounts of unlabeled data from the target domain to improve model adaptation in few-shot settings. We demonstrate self-training to significantly improve with prompt-based fine-tuning~\citep{gao2021making} where we iteratively update a pair of teacher and student models given {\em natural language prompts} and {\em very few labeled examples for the task}. Since the uncertain teacher in few-shot settings produces noisy pseudo-labels, we further use meta-learning to re-weight the pseudo-prompt labels.

%Traditional self-training is quite expensive if we have to update all model parameters. Therefore, we introduce the next technique for lite self-training.

\noindent {\em (b) Light-weight adapter-tuning.} Traditional self-training can be expensive if we have to update all model parameters iteratively. Therefore, we show that we can use a small number of task-specific adapter parameters in the PLM that are updated with few-shot labels, while keeping the large PLM encoder fixed. We demonstrate that light-weight tuning with self-training can match the setting where all model parameters are tuned.  
This enables efficient use of self-training, improves parameter efficiency of the fine-tuning process, and reduces the storage cost of the fine-tuned model since multiple fine-tuned models can now share the same PLM as backbone during inference.

%\noindent {\em (b) Light-weight adapter-tuning.} We introduce a small number of task-specific adapter parameters in the PLM that are updated with few-shot labels, while keeping the large PLM encoder fixed. This reduces the number of tunable parameters during self-training, as well as the storage cost since multiple fine-tuned models can now share the same PLM as backbone during inference. The VRAM consumption could also be reduced as we do not need to keep track of the optimizer states for the frozen parameters.
Consider the following scenario for demonstration, where we want to use RoBERTa-large with $\mathcal{M}=355M$ parameters as the PLM for $\mathcal{T}=100$ tasks. Full fine-tuning for this scenario requires updating and storing $\mathcal{M}\times\mathcal{T}=35.5B$ parameters. Now, consider fine-tuning with \sysname that requires $\mathcal{A}=14M$ (tunable) adapter parameters for every task while keeping the PLM fixed. This results in overall $\mathcal{M}+\mathcal{A}\times\mathcal{T}=1.8B$ parameters, thereby, reducing the overall storage cost by 20x. %$20x$. 

We perform extensive experiments in six natural language understanding tasks to demonstrate the effectiveness of \sysname. We devise a comprehensive evaluation framework considering the variance in few-shot performance of PLMs with different shots, random seeds and splits\footnote{We will release the code and dataset partitions for different shots, seeds and splits for every task to enable reproducability and benchmarking of efficient few-shot language models.}. Results show that \sysname improves over traditional and more recent prompt-based FN  methods by $35\%$ and $6\%$, respectively, with $96\%$ reduction in number of trainable parameters given only $30$ labeled examples for each downstream task. Figure~\ref{fig:key-result} shows the results on MNLI \citep{mnli} as an example.

  


%We develop a resource-efficient method for adapting large language models for tasks that addresses both labeled data-efficiency ({\em C1}) to train PLMs given very few labeled examples and unlabeled data, and parameter-efficiency ({\em C2}) to update only a small number of the tunable model parameters.
%While resource-rich benchmarks like GLUE~\cite{} demonstrate several of the PLMs to outperform human performance for several tasks, the evaluation framework is not quite fair for the humans who can perform complex tasks given only a few demonstrative examples.





% \begin{figure}[hbt]
% \vspace{-0.1in}
% \subfloat[]{
% \begin{minipage}{.49\textwidth}
% \includegraphics[height=1.9in]{figures/open_fig_1_black}
% \label{subfig:twitter}
% \end{minipage}}
% \subfloat[]{
% \begin{minipage}{.49\textwidth}
% \includegraphics[height=1.9in]{figures/open_fig_2}
% \label{subfig:weibo}
% \end{minipage}}


% \caption{\sysname leverages prompt-tuning with unlabeled data for label-efficiency and adapters for reducing tunable model parameters. (a) shows classic tuning, prompt-tuning and \sysname using RoBERTa-large as backbone on MNLI task for a comparison. The red dash line depicts the ceiling performance with full supervision ($400\mathrm{K}$ training labels) with RoBERTa-large.  (b) shows the number of tunable parameters for each tuning method.}

% \end{figure}


% To summarize, we make the following contributions.% in this work.

% \noindent {\bf (a)} We demonstrate the benefits of using self-training with prompts and unlabeled data to adapting large language models in few-shot settings. To this end, we develop a semi-supervised prompt-tuning method, namely \sysname for tuning large language models with access to very few training labels ($K \in \{10, 20, 30\}$) and unlabeled data. \sysname leverages self-training to learn from pseudo prompt-labels and meta-learning for noisy pseudo-label re-weighting.

% \noindent {\bf (b)} We leverage adapters to massively reduce the number of tunable parameters in \sysname with techniques like knowledge distillation to stabilize adapter training for few-shot learning. This allows us to obtain both label- and parameter-efficiency. To the best of our knowledge, this is the first work to study the impact of adapters in the few-shot setting.

% \noindent {\bf (c)} Finally, we perform extensive experiments in six NLU tasks to demonstrate the effectiveness of the above approaches with comprehensive analysis on the trade-off in model size, labeled data- and parameter-efficiency. Given the wide variance in PLM performance in few-shot settings with different shots, random seeds and splits -- we devise a comprehensive framework\footnote{We will release the dataset partitions for different shots, random seeds and splits for every task to enable benchmarking of efficient few-shot language models.} for evaluation.  


% \begin{wrapfigure}{r}{0.4\textwidth}
% \vspace{-1em}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{figures/PromptST.png}
%   \end{center}
%   \caption{Prompt-tuning with $30$ labeled examples for each task aggregated over six NLU tasks with different encoders. The red line depicts the ceiling performance with full supervision ($8K-400K$ training labels) with RoBERTa-large. \sysname uses RoBERTa-large as the base encoder.}
%   \vspace{-1em}
% \end{wrapfigure}



\noindent {\bf Problem statement.} Each downstream task in our framework consists of very few labeled training examples $\mathcal{D}^{Train}_K$ for different shots $K \in \{10, 20, 30\}$ where $|\mathcal{D}^{Train}_K| = K$, unlabeled data $\mathcal{D}^U$ where $\mathcal{D}^{U} \gg \mathcal{D}^{Train}_K$, and a test set $\mathcal{D}^{Test}$.%, and a natural language task prompt {which is a task-specific template}.


%\noindent {\bf Problem statement.} Each task in our framework consists of very few labeled training examples $\mathcal{D}^{Train}_K$ for different shots $K \in \{10, 20, 30\}$ where $|\mathcal{D}^{Train}_K| = K$, unlabeled data $\mathcal{D}^U$ where $\mathcal{D}^{U} \gg \mathcal{D}^{Train}_K$ and a test set $\mathcal{D}^{Test}$, as well as a natural language task prompt.

%Each labeled example consists of {original input sentences with corresponding task prompts.}

%a natural language context, a natural language question, and an answer. \xiaodl{Usually, a general training sample include an input x and a label y. I feel the current definition is more like for QA. We may need a bit explanation here. Additionally, for Figure 2, does it require to a [SEP] between context/question?}

Given the above dataset $\mathcal{D}_K=\mathcal{D}^{Train}_K \cup \mathcal{D}^U$ for a task with shots $K$, a PLM with parameters $\Theta_{\mathrm{PLM}}$ and a loss function $\mathcal{L}$, we want to adapt the model for the few-shot learning task by introducing a small number of tunable model parameters $\psi \ll \Theta_{\mathrm{PLM}}$. 

\vspace{-0.1in}
\section{Background on Model Fine-tuning}\vspace{-0.1in}
\label{subsec:primer}

Given a text sequence ${x}$ or a pair of sequences $\{x_1, x_2\}$ separated by special operators (e.g., {\small [CLS]} and {\small [SEP]}) and a language model encoder $enc (\theta)$ parameterized by $\theta$ -- classic fine-tuning popularized by \citep{BERT} leverages hidden state representation $h_{[CLS]}$ of the sequence(s) obtained from $enc([\text{\small [CLS]}\ x_1\ \text{\small [SEP]}\ x_2\ \text{\small [SEP]}])$ as input to a task-specific head $softmax(W^T \cdot h_{[CLS]})$ for classification, where $W \in \mathbb{R}^{d \times L}$ with $d$ and $L$ representing the hidden state dimension and number of classes respectively, are randomly initialized tunable parameters. In the process it updates both task-specific head $W$ and encoder $\theta$ parameters jointly.

%Given a pair of question $q$ and a passage $p$ in the form of "\texttt{ST} \texttt{[question]} \texttt{[passage]}", the PLM produces contextualized embeddings for all input tokens.
%Specifically, for each token position $t$ in the input,
%the final hidden vector $\hvec_t \in \RR^d$ 
% is the contextualized token embedding.
% The span-begin score is computed as 
% $s_b(i) = \wvec_b^T \hvec_i$ using a weight vector
% $\wvec_b \in \RR^d$.
% The probability for a span start $i$ is $P_b(i) = {\exp(s_b(i)) \over Z_b}$,
% where $Z_b$ is the normalizing factor over all positions.
% The span-end score $s_e(j)$ and probability $P_e(j)$ are defined similarly.
% The probability of an answer span $(i, j)$ is
% $ P(i,j) = P_b(i) P_e(j)$.
% % $ P(i,j) = P_b(i) P_e(j) = {\exp (s_b(i) + s_e(j)) \over Z_b Z_e}$.
% The training is then carried out by maximizing the log-likelihood of the answer span.



% \begin{wrapfigure}{r}{0.35\textwidth}
% \centering
% \vspace{-0.2in}
% \includegraphics[width=1\linewidth]{./figures/only_framework.pdf}
% \caption{The underlined text refers to task prompt of transforming classification into fill-in-mask format. The label words are pre-defined  and used as proxy of original task labels..}\label{fig:example}
% \vspace{-0.0in}
% \end{wrapfigure}


However, this introduces a gap between pre-training and fine-tuning objective with disparate label spaces and additional randomly initiated parameters $W$ introduced for task-specific fine-tuning. This is particularly challenging for few-shot classic fine-tuning, where the limited labeled data is inadequate for adapting the task-specific head and PLM weights effectively. 
Prompt-based FN~\citep{schick-schutze-2021-just, gao2021making} addresses this gap, by re-formulating the objective as a cloze-style auto-complete task. This is done by adding a phrase (also called {\em prompt}) to a sentence like $x_1 =\ $``{\tt \small contains no wit, only labored gags}" in the form of $\Tilde{x} = x_1\ \oplus $ ``{\tt \small It was [MASK]}", where $\oplus$ denotes the concatenation of two strings; and output mappings (also called {\em verbalizers}) from vocabulary $\mathcal{V}$ to the label space $\mathcal{Y}$ like ``{\tt \small \{great, terrible\}}" corresponding to positive and negative classes (refer to Figure~\ref{fig:prompt} for an example).
% The fine-tuning objective of psimilar to that of pre-training is to predict masked tokens given by:
The probability of predicting class $y \in \mathcal{Y}$ is equal to calculating the probability of corresponding label word $v \in \mathcal{V}$:
\begin{equation}
\label{eq:prompt-tune}
\small
%p(\mathrm{[MASK]} = v |\Tilde{x}) = \frac{\exp(\theta_v \cdot h_{\mathrm{[MASK]}})}{\sum_{v' \in V} \exp(\theta_{v'} \cdot h_{\mathrm{[MASK]}})}  
p(\mathrm{[MASK]} = v |\Tilde{x}) = \frac{\exp(W^T_v \cdot h_{\mathrm{[MASK]}})}{\sum_{v' \in V} \exp(W^T_{v'} \cdot h_{\mathrm{[MASK]}})}
\end{equation}
\noindent where  $W_v$ indicates the tunable parameters. Since it is identical to masked language modeling (MLM), $W_v$ is initialized by the pre-trained weights of PLMs.

%\noindent where $V$ is the size of the vocabulary and $W_v$ denotes the pre-softmax vector corresponding to the token $v$. Since this optimization objective directly leverages the pre-trained weights $\theta_v$, it does not introduce any additional task-head parameters.

% \xiaodl{Should we stress randomness of task head? We didn't use $W_v$ here. Is it $\theta_v$?} \yq{I think we also did not introduce $h_{\mathrm{[MASK]}}$.}

% \yq{

% \begin{equation}
% \label{eq:prompt-tune}
% \small
% p(y |\Tilde{x}) = \frac{\exp(p(\mathrm{[MASK]} = v|\Tilde{x}))}{\sum_{v' \in V} \exp(\mathrm{p(\mathrm{[MASK]} = v'|\Tilde{x}))})}  
% \end{equation}

% \noindent where $p(\mathrm{[MASK]} = v|\Tilde{x}))$ denotes the pre-softmax vector corresponding to the token $v$ via the pre-trained language model head. Since this prediction directly leverages the pre-trained weights, it does not introduce any additional task-head parameters.}

{\em In this work, we demonstrate that lite self-training with unlabeled data can significantly improve prompt fine-tuning of large language models in few-shot settings.}

%given by the following parameterization:

%\begin{equation}
%\psi \leftarrow argmin_{\Psi'}\  \mathcal{L} (\mathcal{D}_K; \Theta_{\mathrm{PLM}}, \psi')
%\end{equation}



%Given the variance in few-shot model performance across different seeds and splits of the data, for each $k$-shot setting, we provide $5$ training splits (satisfying the subset inclusion criteria above for each split across multiple shots) and a single test set for reporting both the mean and variance in model performance.



% take figure 3 to appendix 

==> subfiles/methodology_backup.tex <==
\vspace{-0.15in}
\section{Methodology}
\vspace{-0.15in}
\subsection{Primer}
\label{subsec:primer}
\vspace{-0.5em}
\noindent {\bf Self-training.} We leverage self-training as the backbone of our framework. The algorithm is composed of two phases that are executed iteratively until convergence. In the first phase, we train teacher model on the few-shot labeled set $\mathcal{D}^{Train}_K$ to estimate the parameters of a {\em teacher} model. In the second phase, we leverage the teacher model to infer pseudo-labels for the unlabeled set $\mathcal{D}^u$ and train a {\em student} model to mimic the teacher's predictions for the task label. Finally, the teacher model is updated with the student model's parameters and above steps are repeated until convergence. 
%
% The optimization objective for the above self-training process can be formulated as:
%
% \begin{equation}
%     \label{eq:st}
%     min_\theta\ \mathbb{E}_{x_l, y_l \in \mathcal{D}^{Train}_K} [-log\ p (y_l|x_l;\theta)] +
%     \lambda\ \mathbb{E}_{x_u \in \mathcal{D}^u}  \mathbb{E}_{y_u \sim p(y|x_u;\theta^*)} [-log\ p (y_u|x_u;\theta)]
% \end{equation}
%
% \noindent where $p(y|x;\theta)$ is the conditional distribution under model parameters $\theta$. $\theta^*$ is given by the model parameters from the last iteration and fixed in the current iteration. 
%
Similar optimization have been used recently in variants of self-training for neural sequence generation~\citep{he2019revisiting}, data augmentation~\citep{xie2019unsupervised} and knowledge distillation~\citep{mukherjee-hassan-awadallah-2020-xtremedistil}. 
% 
Due to the noisy nature of pseudo-labels, the above self-training process may result in gradual drifts~\cite{DBLP:conf/iclr/ZhangBHRV17}. To address this, we train the student model to explicitly account for the teacher's confidence and uncertainty on the generated pseudo-labels with a re-weighting mechanism leveraging meta-learning (discussed in Section~\ref{sec:reweight}). 

\noindent {\bf Prompt-tuning.} Given a text sequence ${x}$ or a pair of sequences $\{x_1, x_2\}$ separated by special operators (e.g., {\small [CLS]} and {\small [SEP]}) and a language model encoder $enc (\theta)$ parameterized by $\theta$ -- classic fine-tuning popularized by \citep{BERT} leverages hidden state representation $h_{[CLS]}$ of the sequence(s) obtained from $enc([\text{\small [CLS]}\ x_1\ \text{\small [SEP]}\ x_2\ \text{\small [SEP]}])$ as input to a task-specific head $softmax(W \cdot h_{[CLS]})$ for classification, where $W \in \mathbb{R}^{d \times L}$ with $d$ and $L$ representing the hidden state dimension and number of classes respectively. In the process it updates both task-specific head $W$ and encoder $\theta$ parameters jointly.

%Given a pair of question $q$ and a passage $p$ in the form of "\texttt{ST} \texttt{[question]} \texttt{[passage]}", the PLM produces contextualized embeddings for all input tokens.
%Specifically, for each token position $t$ in the input,
%the final hidden vector $\hvec_t \in \RR^d$ 
% is the contextualized token embedding.
% The span-begin score is computed as 
% $s_b(i) = \wvec_b^T \hvec_i$ using a weight vector
% $\wvec_b \in \RR^d$.
% The probability for a span start $i$ is $P_b(i) = {\exp(s_b(i)) \over Z_b}$,
% where $Z_b$ is the normalizing factor over all positions.
% The span-end score $s_e(j)$ and probability $P_e(j)$ are defined similarly.
% The probability of an answer span $(i, j)$ is
% $ P(i,j) = P_b(i) P_e(j)$.
% % $ P(i,j) = P_b(i) P_e(j) = {\exp (s_b(i) + s_e(j)) \over Z_b Z_e}$.
% The training is then carried out by maximizing the log-likelihood of the answer span.
\begin{wrapfigure}{r}{0.35\textwidth}
\centering
\vspace{-0.2in}
\includegraphics[width=1\linewidth]{./figures/only_framework.pdf}
\caption{Prompt-tuning with unlabeled data and adapters make efficient few-shot learners: \sysname  Architecture.}\label{fig:framework}
\vspace{-0.2in}
\end{wrapfigure}


% \begin{wrapfigure}{r}{0.35\textwidth}
% \centering
% \vspace{-0.2in}
% \includegraphics[width=1\linewidth]{./figures/only_framework.pdf}
% \caption{The underlined text refers to task prompt of transforming classification into fill-in-mask format. The label words are pre-defined  and used as proxy of original task labels..}\label{fig:example}
% \vspace{-0.0in}
% \end{wrapfigure}


However, this introduces a gap between pre-training and fine-tuning objective with disparate label spaces and additional softmax parameters $W$ introduced for task-specific fine-tuning. This is particularly challenging for few-shot classic fine-tuning, where the limited labeled data is inadequate for adapting the task-specific head and PLM weights effectively. 
Prompt-based fine-tuning~\citep{gao2021making,DBLP:journals/corr/abs-2101-00190,DBLP:journals/corr/abs-2104-08691,liu2021gpt} addresses this gap, by re-formulating the objective as a cloze-style auto-complete task. For instance, we can add a phrase (also called {\em prompt}) to a sentence like $x_1 =\ $``{\tt \small contains no wit, only labored gags}" in the form of $\Tilde{x} = x_1\ \oplus $ ``{\tt \small It was [MASK]}" -- where the fine-tuning objective similar to that of pre-training is to predict the masked tokens given by:
\begin{equation}
\label{eq:prompt-tune}
\small
p(\mathrm{[MASK]} = v |\Tilde{x}) = \frac{\exp(\theta_v \cdot h_{\mathrm{[MASK]}})}{\sum_{v' \in V} \exp(\theta_{v'} \cdot h_{\mathrm{[MASK]}})}  
\end{equation}
\noindent where $V$ is the size of the vocabulary and $W_v$ denotes the pre-softmax vector corresponding to the token $v$. Since this optimization objective directly leverages the pre-trained weights $\theta_v$, it does not introduce any additional task-head parameters.

{\em In this work, we demonstrate that self-training with unlabeled data can significantly improve prompt-tuning of large language models in few-shot settings.}

%In this work, we adopt the same set of pattern templates and verbalizers as in
%~\citep{gao2021making} for SST-2 and MNLI with 
%different PLMs. 


%\subsection{Few-shot Fine-tuning}


%\subsection{Lightweight Few-shot Model Tuning}




\vspace{-0.5em}
\subsection{Lightweight Prompt Adapter tuning}
\label{subsec:prompt-adapter}\vspace{-0.5em}
The predominant methodology for task adaptation is to tune all of the trainable parameters of the PLMs for every task. This raises significant resource challenges both during training and deployment. A recent study~\citep{aghajanyan2020intrinsic} show that PLMs have a low instrinsic dimension that can match the performance of the full parameter space. 
%Inspired by this observation, we wonder whether we could tuning only a small set of parameters when adapting to downstream tasks with only very few labeled samples. 
To adapt PLMs for downstream tasks with a small number of parameters, adapters~\citep{houlsby2019parameter} have recently been introduced as an alternative approach for lightweight tuning. Adapters have been shown to match the PLM performance in {fully supervised settings with thousands of training labels in classic fine-tuning}. {\em In contrast, this is the first work to study the role of adapters in few-shot prompt-tuning.} We explore different design and placement choices of adapters in few-shot settings and investigate the performance gap with fully supervised as well as fully tunable parameter space. 

\begin{wrapfigure}{r}{0.35\textwidth}
\vspace{-1em}
 	\centering
   	\includegraphics[width=1\linewidth]{./figures/adapter.pdf}\vspace{-0.5em}
 	  	\caption{\sysname explores several adapter placement choices (numbered positions in left) in standard Transformer architecture, with adapter design shown in right.}
 	 	 	\label{fig:adapter}
\vspace{-1.5em}
\end{wrapfigure}

The adapter tuning strategy judiciously introduces new parameters into the original PLMs.  In contrast to standard prompt-tuning that updates all the PLM parameters $\Theta_{\mathrm{PLM}}$, prompt-adapter tuning only updates the newly introduced adapter parameters as well as the (masked) language model head of the PLM (jointly denoted as $\psi$),  while keeping the remaining parameters of the original network frozen. \yq{Adapters usually consist of two fully connected layers as shown in Figure~\ref{fig:adapter}, where a feedforward layer down projects representations to a low dimensional space $d$ (referred as the bottleneck dimension), and another feedforward layer up projects the low-dimensional features back to the original dimension.  However, these newly-inserted parameters can cause divergence resulting in upto $20\%$ performance degradation in few-shot settings (discussed in Section~\ref{subsec:adapter}). To handle this issue, we adopt a skip-connection design where the adapter parameters are initialized with zero-mean small gaussian noise. }

\yq{\noindent\textbf{Practical benefits of lite tuning.} The most significant benefit of lightweight adapter tuning comes from the reduction in memory and storage usage. For a Transformer, The VRAM consumption could be significantly reduced as we do not need to keep track of the optimizer states for the frozen parameters. For storage usage, we also reduce the checkpoint size by 25x (from 355MB to 14MB) since we store adapter instead of entire PLM, largely benefit deployment. }

Prior work on lightweight adaptation~\cite{cai2020tinytl} tune bias or embeddings of transformers in fully-supervised settings for improving parameter-efficiency with minimal performance loss. However, for few-shot settings, we demonstrate that adapter placement is critical to bridge the performance gap with that of a fully tunable model. To this end, we explore several choices of adapter placement (refer to Figure~\ref{fig:adapter}) corresponding to the most important transformer modules, namely, 
%
%Even though many lightweight studies~\cite{} show tuning of bias or embedding component could achieve good performance in resource rich scenario, those findings are not valid based on our empirical studies for few-shot learning. For example, only tuning bias or continuous prompt could lead to a gap of more than  10\% compared to full model tuning.  
%
%Therefore, we need to identify most important modules in few-shot tuning. The PLMs usually include four important modules: 
embedding, intermediate feedforward, output feedforward and attention module in {\em every layer} of the transformer model. Based on empirical experiments (refer to Section~\ref{subsec:adapter}) across six diverse NLU tasks, we observe the feedforward output and attention modules to be the most important components for parameter-efficient adaption in few-shot settings.

%in experimental section~\ref{subsec:adapter} and get the consistent finding: the Feedforward-output and Attention modules are most effective in few-shot tuning despite data sample size and tasks. Such a pilot study instructs us to insert Adapter into these two modules to for downstream task adaptations.

Given the above adapter design and placement of choice with parameters $\psi$, the dataset $\mathcal{D}_K$ with shots $K$, a pre-trained language model encoder $enc$ with parameters $\Theta_{\mathrm{PLM}}$, where $\Theta_{\mathrm{PLM}} \gg \psi$, we want to perform the following optimization for efficient model adaptation:
\begin{equation}
\psi \leftarrow \argmin_{\psi}\  \mathcal{L} (\mathcal{D}_k; \Theta_{\mathrm{PLM}}, \psi)
\end{equation}
\vspace{-0.2in}
\subsection{Few-shot Semi-supervised Prompt-tuning}\vspace{-0.5em}
We adopt a pre-trained language model (e.g., BERT~\citep{BERT}, RoBERTa~\citep{RoBERTa}, T5~\citep{T5}) as the {\em shared encoder} for both the student and teacher model for self-training. We introduce {\em tunable adapter parameters in each} (following discussions in Section~\ref{subsec:prompt-adapter}) and keep the shared encoder frozen (that is not updated) during training. Now, given few-shot labeled examples, we first leverage prompt-tuning (Equation~\ref{eq:prompt-tune}) to tune the teacher adapter and the language model head for the underlying task. The tuned teacher is used to pseudo-label the unlabeled data $\mathcal{D}^u$. In the most general version of self-training, the student is used to mimic the teacher predictions on the pseudo-labeled data. However, the few-shot setting results in a noisy teacher resulting in error propagation from noisy labels~\citep{DBLP:conf/iclr/ZhangBHRV17,ruder2018strong}. 

Training deep networks with noisy labels has been studied in settings like weak supervision~\cite{} and learning from noisy user interactions~\cite{}. Notably several of these works use auxiliary information for error estimation and re-weighting in the form of source trustworthiness~\cite{}, label corruption matrices~\cite{}, etc. A popular line of work in this setting include meta-learning~\cite{} to re-weight the noisy labels. In this work, we adopt and adapt the meta-learning approach to re-weight noisy prompt labels in few-shot setting.







\vspace{-0.5em}
\subsubsection{Re-weighting Noisy Prompt Labels}
\label{sec:reweight}
\vspace{-0.5em}
Consider $\widetilde{\mathcal{D}}^{Train}_K=\{\widetilde{x}^l, \widetilde{y}^l\}$ to be the few-shot labeled data and $\widetilde{\mathcal{D}}^U=\{\widetilde{x}_u\}$ to be the unlabeled data, where we transform the input sequences $X$ to cloze-style input $\widetilde{X}$ containing a single mask and $\widetilde{\mathcal{Y}}: {\mathcal{Y}} \rightarrow \mathcal{V}$ following the prompting strategy outlined in Section~\ref{subsec:primer}. We use the same pattern templates and verbalizers (output mapping from the task-specific labels $\mathcal{Y}$ to single tokens in the vocabulary $\mathcal{V}$) from traditional prompt-tuning works~\citep{gao2021making,schick-schutze-2021-just}.




% To mitigate error propagation from noisy pseudo-labeled sequences from the teacher, we leverage meta-learning to adaptively re-weight them based on the student model loss on the sampled validation set as our meta-objective. The validation set is obtained by our adaptive sampling strategy from the previous step. In contrast to prior work on instance-level image and text classification, %sequence labeling operates on discrete text sequences as input and assigns labels to each token in the sequence. Since teacher predictions vary for different slot labels and types, 
% we adapt the meta-learning framework to re-weight noisy pseudo-labeled samples at a token-level resolution for the sequence labeling task.  

Consider $\{\hat{y}^{(t)}_{n}\}_{n=1}^N$ to be the pseudo prompt-labels (for the masked tokens in $\widetilde{x}^u_{n} \in \widetilde{X}$) from the teacher in the $t$-th iteration where $N$ is the number of unlabeled instances. In self-training, the student model is trained to mimic the teacher predictions on the transfer set. Consider $\mathcal{L}(\hat{y}^{(t)}_{n}, \mathrm{enc}(\widetilde{x}^u_{n}; \Theta_{\mathrm{PLM}}, \psi^{(t)}_{\mathrm{stu}}))$ to be the loss of the student model with parameters $(\Theta_{\mathrm{PLM}}, \psi^{(t)}_{\mathrm{stu}})$ on the pseudo-labeled data in the $t$-th iteration, where $\Theta_{\mathrm{PLM}}$ and $\psi_{\mathrm{stu}}$ represent the PLM and the adapter parameters respectively. The student update step (with step size $\alpha$) can be formalized as:
\vspace{-0.2em}
\begin{equation}
\small
\hat{\psi}^{(t)}_{\mathrm{stu}} = \hat{\psi}^{(t-1)}_{\mathrm{stu}} - \alpha \triangledown \big (  \frac{1}{N}  \sum_{i=1}^N \mathcal{L}(\hat{y}^{(t)}_{i}, \mathrm{enc}(x^u_{i}; \Theta_{\mathrm{PLM}}, \hat{\psi}^{(t-1)}_{\mathrm{stu}}) \big ).
\end{equation}
In order to reduce drift from noisy pseudo-labels, we leverage meta-learning to re-weight them based on the student model loss on the validation set as our meta-objective. 

A typical challenge in few-shot settings is the lack of a separate validation set. In the spirit of {\em true} few-shot learning, we use only the available few-shot labeled examples $\widetilde{\mathcal{D}}^{Train}_K$ as the validation set for meta-learning of the student model. This poses an interesting challenge of preventing label leakage, since the base prompt-teacher model is also fine-tuned on the same labeled set.  
%
%\noindent \textbf{Student Adapter Re-initialization.} Even though iterative tuning on labeled data and pseudo-labeled data brings improvements, such a procedure also poses challenges on how to keep labeled data held-out to student model for pseudo-labeled data re-weighting. 
To address this issue, we {\em re-initialize the student adapter parameters} every time at the start of each self-training iteration to mitigate interference with labeled data. Note that the student and teacher model share the encoder parameters $\Theta_{\mathrm{PLM}}$ that are always kept frozen and not updated during training. 
%We demonstrate the impact of this choice with ablation study in experiments. , which is given few-shot labeled dataset $\widetilde{\mathcal{D}}^{Train}_K$

\yq{To handle error-propagation, we leverage meta-learning to re-weight noisy prompt labels on the pseudo-labeled data. The intuition of meta re-weighting is to measure the impact or weight of a pseudo-labeled example given by its performance on the validation set ($\widetilde{\mathcal{D}}^{Train}_K$ in our work). To this end, we leverage the idea of weight perturbation~\citep{koh2017understanding, ren2018learning} to set the weight of pseudo-labeled example $(\widetilde{x}^u_{i}, \hat{y}^{(t)}_{i})$ to $\epsilon^{(t)}_{i}$ at iteration $t$ as:}
\begin{equation}
\small
    \hat{\psi}^{(t)}_{\mathrm{stu}} (\epsilon) = \hat{\psi}^{(t-1)}_{\mathrm{stu}} - \alpha \triangledown  \big (  \frac{1}{N} \sum_{i=1}^{N} [\epsilon^{(t)}_{i} \cdot \mathcal{L}(\hat{y}^{(t)}_{i}, \mathrm{enc}(\widetilde{x}^u_{i}; \Theta_{\mathrm{PLM}},  \hat{\phi}^{(t-1)}_{\mathrm{stu}}))] \big ).
\end{equation}
\yq{Weight perturbation is used to discover data points that are most important to improve the model performance on the validation set.  The optimal value for the perturbation $\epsilon^{(t)*}_{i}$ can be obtained via the student model loss minimization on the validation set at iteration $t$ as:}
\begin{equation}
\small
\epsilon^{(t)*}_{i} = \argmin_{\epsilon_{i}} \frac{1}{|\widetilde{\mathcal{D}}^{Train}_K|}  \sum_{i=1}^{|\widetilde{\mathcal{D}}^{Train}_K|} \mathcal{L}({y}_{i}, \mathrm{enc}(x_{i}; \Theta_{\mathrm{PLM}}, \hat{\psi}^{(t)}_{stu}(\epsilon_{i}))
\end{equation}
 To obtain a cheap estimate of the meta-weight at step $t$, we take a single gradient descent step on a mini-batch $\widetilde{\mathcal{D}}^{(t)} \in \widetilde{\mathcal{D}}^{Train}_K$ as:
\begin{equation}
\small
    u_{i}^{(t)} = -\frac{\partial}{\partial{\epsilon_{i}}}  \bigg ( \frac{  \sum_{i=1}^{|\widetilde{\mathcal{D}}^{(t)}|}  \mathcal{L}(y_{i}, \mathrm{enc}(\widetilde{x}_{}; \Theta_{\mathrm{PLM}},  \hat{\psi}^{(t)}_{stu} (\epsilon)))}{{|\widetilde{\mathcal{D}}^{(t)}|}} \bigg) \bigg|_{\epsilon_{i}^{(t)} = 0}
\end{equation}
\yq{The weight  $w_{i}^{(t)}$  of $(\widetilde{x}^u_{i}, \hat{y}^{(t)}_{i})$ at iteration $t$ can be set to be proportional to the negative gradient $u_{i}^{(t)}$ to reflect the importance of pseudo-labeled samples. The samples with negative weights are filtered out since they could potentially degrade the student performance. Finally, we update the student adapter parameters $\psi_{\mathrm{stu}}$ while accounting for re-weighting as:}
\begin{equation}
\small
\label{Eq:meta_update}
    \hat{\psi}^{(t)}_{stu} = \hat{\psi}^{(t-1)}_{stu} - \alpha  \triangledown \big ( \frac{1}{N}  \sum_{i=1}^{N} [w_{i}^{(t)} \cdot \mathcal{L}(\hat{y}^{(t)}_{i}, \mathrm{enc}(\widetilde{x}^u_{i}; \Theta_{\mathrm{PLM}}, \hat{\psi}^{(t-1)}_{\mathrm{stu}}))] \big ). \vspace{-0.1in}
\end{equation}

% as:

% \begin{equation}
%     w_{m, n} = \frac{w_{m, n}}{\sum_{m=1}^M\sum_{n=1}^N w_{m, n}}
% \end{equation}



%\begin{remark}
%The contributions of pseudo-labeled data need to be estimated with the help of hold-out set. To ensure labeled data is hold-out for student, the student needs to be \textbf{re-initialized} after every cycle of self-training. 
%\end{remark}
 
\vspace{-0.5em}
\subsubsection{Knowledge Distillation as Warmup}
\vspace{-0.5em}

Meta re-weighting mechanism leverages gradient as a proxy to estimate the weight of noisy pseudo labels. However, the gradients of adapters parameters $\psi$ are not stable in the early stages of training due to random initialization. This instability issue is further exacerbated with adapter tuning that usually requires a larger learning rate~\citep{pfeiffer2020AdapterHub}. Therefore, to stabilize adapter tuning, we propose a warmup training stage via knowledge distillation~\citep{hinton2015distilling}. To this end, we first tune adapter parameters via knowledge distillation loss and then we continue self-training with re-weighting via Eq.~\ref{Eq:meta_update}. Since the re-weighting procedure requires held-out validation set (few-shot training examples in our setting), we do not use labeled data in knowledge distillation while using only the consistency loss between teacher model $(\Theta_{\mathrm{PLM}}, \hat{\psi}_{\mathrm{tea}})$ and student model $(\Theta_{\mathrm{PLM}}, \hat{\psi}_{\mathrm{stu}})$ on unlabeled data as follows.
\begin{equation}
\small
\label{Eq:meta_update}
    \hat{\psi}_{stu}  \leftarrow \argmin_{\hat{\psi}_{stu}} \infdiv{f(\widetilde{x}^u; \Theta_{\mathrm{PLM}}, \hat{\psi}_{\mathrm{tea}})}{f(\widetilde{x}^u; \Theta_{\mathrm{PLM}}, \hat{\psi}_{\mathrm{stu}}) }. 
\end{equation}
We further validate the effectiveness of knowledge distillation for warmup with ablation analysis. 
\vspace{-0.5em}
\subsection{Lite Self-training for \sysname}
\label{sec:teacher_finetune}\vspace{-0.5em}
We first prompt-tune the teacher adapter with few-shot labeled data and leverage the teacher model to infer pseudo-prompt labels on unlabeled data. The noisy pseudo-labeled samples are further re-weighted via meta-learning.  Since we follow true few-shot learning setting without any development set, we train the models for a pre-defined number ($T=1000$) of self-training iterations. Finally, we assign the trained student adapter to be the new teacher adapter (i.e., $\psi_{\mathrm{tea}} = \psi^{(T)}_{\mathrm{stu}}$) and repeat the above steps till convergence. The overall training procedure is summarized in Algorithm~\ref{alg} (Appendix~\ref{sec:alg}). Throughout the training, we keep the shared student and teacher encoder parameters frozen and only update the adapter parameters along with the corresponding language model heads.

%It is worth noting that one of key steps in our self-training framework is to utilize the labeled data $(\{x^l_{n},y^l_{n}\})$ to fine-tune the new teacher model $\psi_{\mathrm{tea}}, i.e., \psi^{(T)}_{\mathrm{stu}}$) in every self-training session. Such a step is different with conventional self-training framework, which either leverages labeled data for initial teacher fine-tuning or combine labeled data with unlabeled data for  joint training of student model.  The iterative usage of labeled data and labeled data  procedure is similar to seeking a better teacher initialization before further prompt tuning on $(\{x^l_{n},y^l_{n}\})$ and such a procedure plays a key role in improving teaching model and  pseudo labels.

%
%We explore the effectiveness of this step with an ablation study in experiments. 
%



%This de-coupled view enables the models to efficiently use the labeled training data. %Prior work on self-training for neural sequence generation~\citep{he2019revisiting} demonstrate improvement on further fine-tuning the student model afte
% This raises the question if we can further improve the student model performance by fine-tuning on the labeled data while accounting for the separation in its view of the training labels. 


%
%To this end, at the end of every self-training iteration, we further utilize the labeled data $(\mathbf{X}^l,\mathbf{Y})$ to fine-tune the student model $f(\cdot, \theta_{stu}^{(t)})$ with standard supervised cross-entropy loss minimization. In order to be still able to use this labeled data as a validation set in the next self-training iteration and not explicitly leak the labels to the model, we {\em re-initialize the student model} at the beginning of the self-training iteration. We explore the effectiveness of this step as an ablation study in our experiments. The overall training procedure is summarized in Algorithm~\ref{alg}.



%With effective data selection, the student model is capable of achieving good performance even without using any labeled data for training purpose. Such a mechanism is effective in the extreme low resource setting like hundreds of labels. However, we wonder whether the discarded valuable information from labeled data can help boost the model performance.  Such an intuition is validated by the experiments in the section~\ref{sec:ablation_study}. 


%To take better advantage of given labeled data, we propose a very simple yet effective step: fine-tune student model $f(\cdot, \theta_{stu})$ on labeled data $(\mathbf{X}^l,\mathbf{Y})$. Because we need to hold-out given labeled data for student model to ensure accurate estimate of contribution of pseudo-labeled data, the training on labeled data can only be conducted after end of self-training round.  





% \subsection{MetaST Framework}
% \begin{itemize}
%     \item hard pseudo labels
%     \item re-initialize student
%     \item data selection
%     \item fine-tune student on clean labeled set 
% \end{itemize}










